Silicide-based Josephson field effect transistors for superconducting qubits

Scalability in the fabrication and operation of quantum computers is key to move beyond the NISQ era. So far, superconducting transmon qubits based on aluminum Josephson tunnel junctions have demonstrated the most advanced results, though this technology is difficult to implement with large-scale facilities. An alternative "gatemon" qubit has recently appeared, which uses hybrid superconducting/semiconducting (S/Sm) devices as gate-tuned Josephson junctions. Current implementations of these use nanowires however, of which the large-scale fabrication has not yet matured either. A scalable gatemon design could be made with CMOS Josephson Field-Effect Transistors as tunable weak link, where an ideal device has leads with a large superconducting gap that contact a short channel through high-transparency interfaces. High transparency, or low contact resistance, is achieved in the microelectronics industry with silicides, of which some turn out to be superconducting. The first part of the experimental work in this thesis covers material studies on two such materials: $\text{V}_3\text{Si}$ and PtSi, which are interesting for their high $T_\text{c}$, and mature integration, respectively. The second part covers experimental results on 50 nm gate length PtSi transistors, where the transparency of the S/Sm interfaces is modulated by the gate voltage. At low voltages, the transport shows no conductance at low energy, and well-defined features at the superconducting gap. The barrier height at the S/Sm interface is reduced by increasing the gate voltage, until a zero-bias peak appears around zero drain voltage, which reveals the appearance of an Andreev current. The successful gate modulation of Andreev current in a silicon-based transistor represents a step towards fully CMOS-integrated superconducting quantum computers.

==> pgflibraryshapes.gates.superconducting.code.tex <==

\pgfdeclareshape{JJ}
{
  \inheritsavedanchors[from=rectangle ee]
  \inheritanchor[from=rectangle ee]{center}
  \inheritanchor[from=rectangle ee]{north}
  \inheritanchor[from=rectangle ee]{south}
  \inheritanchor[from=rectangle ee]{east}
  \inheritanchor[from=rectangle ee]{west}
  \inheritanchor[from=rectangle ee]{north east}
  \inheritanchor[from=rectangle ee]{north west}
  \inheritanchor[from=rectangle ee]{south east}
  \inheritanchor[from=rectangle ee]{south west}
  \inheritanchor[from=rectangle ee]{input}
  \inheritanchor[from=rectangle ee]{output}
  \inheritanchorborder[from=rectangle ee]

  \backgroundpath{
	% Draw cross
	\pgf@process{\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@process{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y

    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}

	% Draw wire
	\pgfpointscale{.5}{\pgfpointadd{\pgfqpoint{\pgf@xa}{\pgf@ya}}{\pgfqpoint{\pgf@xa}{\pgf@yb}}}
	\advance\pgf@x by-.5\pgflinewidth
    \pgfpathmoveto{\pgfqpoint{\pgf@x}{\pgf@y}}
	\pgfpointscale{.5}{\pgfpointadd{\pgfqpoint{\pgf@xb}{\pgf@ya}}{\pgfqpoint{\pgf@xb}{\pgf@yb}}}
	\advance\pgf@x by+.5\pgflinewidth
    \pgfpathlineto{\pgfqpoint{\pgf@x}{\pgf@y}}
  }
}

\pgfdeclareshape{JJcap}
{
  \inheritsavedanchors[from=rectangle ee]
  \inheritanchor[from=rectangle ee]{center}
  \inheritanchor[from=rectangle ee]{north}
  \inheritanchor[from=rectangle ee]{south}
  \inheritanchor[from=rectangle ee]{east}
  \inheritanchor[from=rectangle ee]{west}
  \inheritanchor[from=rectangle ee]{north east}
  \inheritanchor[from=rectangle ee]{north west}
  \inheritanchor[from=rectangle ee]{south east}
  \inheritanchor[from=rectangle ee]{south west}
  \inheritanchor[from=rectangle ee]{input}
  \inheritanchor[from=rectangle ee]{output}
  \inheritanchorborder[from=rectangle ee]

  \backgroundpath{
	% Draw cross and box
	\pgf@process{\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@process{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y

    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}

    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
  }
}


==> tikzlibrarycircuits.superconducting.code.tex <==
\usetikzlibrary{circuits}

\usepgflibrary{shapes.gates.superconducting}

%
% Ideal Josephson junction (cross)
%
\tikzset{
    circuit declare symbol=JJ,
    set JJ graphic={
        circuit symbol lines,
        circuit symbol size=width 2 height 2,
        transform shape,
        shape=JJ
    }
}

%
% Josephson junction with an intrinsic capacitance (boxed cross)
%
\tikzset{
    circuit declare symbol=JJ cap,
    set JJ cap graphic={
        circuit symbol lines,
        circuit symbol size=width 2 height 2,
        transform shape,
        shape=JJcap
    }
}

